Learning Multiple Object States from Actions via Large Language Models

Recognizing the states of objects in a video is crucial in understanding the scene beyond actions and objects. For instance, an egg can be raw, cracked, and whisked while cooking an omelet, and these states can coexist simultaneously (an egg can be both raw and whisked). However, most existing research assumes a single object state change (e.g., uncracked -> cracked), overlooking the coexisting nature of multiple object states and the influence of past states on the current state. We formulate object state recognition as a multi-label classification task that explicitly handles multiple states. We then propose to learn multiple object states from narrated videos by leveraging large language models (LLMs) to generate pseudo-labels from the transcribed narrations, capturing the influence of past states. The challenge is that narrations mostly describe human actions in the video but rarely explain object states. Therefore, we use the LLMs knowledge of the relationship between actions and states to derive the missing object states. We further accumulate the derived object states to consider past state contexts to infer current object state pseudo-labels. We newly collect a dataset called the Multiple Object States Transition (MOST) dataset, which includes manual multi-label annotation for evaluation purposes, covering 60 object states across six object categories. Experimental results show that our model trained on LLM-generated pseudo-labels significantly outperforms strong vision-language models, demonstrating the effectiveness of our pseudo-labeling framework that considers past context via LLMs.

==> sec/0_abstract_old.tex <==
\begin{abstract}
% 70-150 words
% Temporally localizing the presence of object states in videos is crucial in understanding human activities beyond actions and objects. Object states a

Recognizing different states of objects through the scene is crucial in understanding human activities beyond actions and objects. However, previous research assumes unidirectional state changes (\eg unpeeled → peeled) and overlooks multiple perspectives. In this work, we propose to formulate object state recognition as a multi-label frame-wise classification task, offering comprehensive state understanding, flexibility in state changes, and reduced ambiguity. The challenge of this task is to collect labor-intensive multi-label annotation for training data.
To address this, we propose a framework that utilizes large language models (LLMs) to generate object state pseudo-labels from action information included in narrations of instructional videos. Our observation is that LLMs include world knowledge on the relationship between actions and their resulting object states, and can infer the presence of multiple object states from past action sequences. 
We evaluate our method with our newly collected Multiple Object States Transition (MOST) dataset including dense temporal annotation of 60 object state categories.
Our model trained by the generated pseudo-labels demonstrates significant improvement of over 29\% in mAP against strong zero-shot vision-language models, showing the effectiveness of explicitly extracting object state information from actions through LLMs.

% Original Abstract
% Temporally localizing the presence of object states in videos is crucial in understanding human activities beyond actions and objects.
% This task has suffered from a lack of training data due to object states' inherent ambiguity and variety.
% To avoid exhaustive annotation, learning from transcribed narrations in instructional videos would be intriguing.
% However, object states are less described in narrations compared to actions, making them less effective.
% In this work, we propose to extract the object state information from action information included in narrations, using large language models (LLMs).
% Our observation is that LLMs include world knowledge on the relationship between actions and their resulting object states, and can infer the presence of object states from past action sequences.
% The proposed LLM-based framework offers flexibility to generate plausible pseudo-object state labels against arbitrary categories.
% We evaluate our method with our newly collected Multiple Object States Transition (MOST) dataset including dense temporal annotation of 60 object state categories.
% Our model trained by the generated pseudo-labels demonstrates significant improvement of over 29\% in mAP against strong zero-shot vision-language models, showing the effectiveness of explicitly extracting object state information from actions through LLMs.
\end{abstract}

==> sec/1_introduction_old.tex <==
\section{Introduction}
\label{sec:intro}

% タスクの導入
What do we need to understand in a scene of cooking an omelet?
Actions and objects involved in the scene, like ``crack eggs into a bowl'' are some of the key elements, but that is not all.
As the scene progresses, objects undergo multiple state changes triggered by human actions.
For example, when one cracks an egg and then whisks it, the {\it whole} egg becomes {\it cracked}, and then becomes {\it whisked} once the action is accomplished, while it remains {\it raw} during these actions.
In addition to actions and objects, it is important to understand how the state of objects actually changes as a result of the actions, which is necessary for various domains such as cooking~\cite{nishimura2021state}, assembly~\cite{damen2016you,sener2022assembly101}, and robotics~\cite{koppula2013anticipating}.

\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{fig/teaser.pdf}
    % \caption{Generating pseudo-object state labels from narration of instructional videos. We propose to infer object states from relatively abundant action information in narration using Large Language Models (LLMs) (left). Inferred action and object state information is then matched with video frames via vision-language models to assign binary labels for each object state (right).}
    \caption{We propose to generate pseudo-object state labels from relatively abundant action information included in narration using LLMs (top). Inferred pseudo-labels are used to train a frame-wise object state classifier (bottom).}
    \label{fig:teaser}
\end{figure}

% 問題設定の背景
Several studies have investigated the recognition of object state changes before and after a specific action in videos. These studies typically assume a unidirectional state change within a video (\eg unboiled egg $\rightarrow$ boiled egg) and learn to recognize three mutually exclusive stages: \textit{initial state}, \textit{action (transitioning state)}, and \textit{end state}. However, this approach has limitations. It does not consider the fact that object states can be represented from multiple perspectives and fails to take into account different aspects of objects. For example, what if an egg has already been cracked before boiling it? The outcome of boiling an egg with and without the eggshell would be different, but the one-way state change model only consider whether the object reaches to the boiled state or not. This neglects the important difference of whether the egg has a shell or not.

% If the system does not assume a one-way state change, it needs to be capable of recognizing multiple object states and determining whether each state applies to the object at any given time. For instance, a whisked egg might later be heated and solidified, which is no longer a liquid whisked state.

% has the following problems:
% \begin{itemize}
%     \item It overlooks the representability of object states from multiple perspectives and fails to handle the occurrence of simultaneous state changes (\eg, an egg can be whisked and combined with milk simultaneously).
%     \item It does not clearly define the scope of meaning implied by a certain state representation, particularly when multiple state changes occur (\eg, a sliced apple would no longer be sliced if a mixer was applied but would be kept sliced if it was just heated).
% \end{itemize}

To this end, we propose to formulate an object state recognition as a multi-label frame-wise classification task, addressing videos that may include several state changes of a particular object. We consider about 10 state classes per objects which are pre-defined by their scope of meaning in a text to avoid ambiguity, and the task is to predict whether each state class is positive or negative for each video frame. This formulation provides the following merits:
(i) \textbf{Comprehensive State Representation}: It allows for the simultaneous capture of multiple possible states of an object, providing a more nuanced understanding of the object's condition at each frame.
(ii) \textbf{Flexibility in State Changes}: This approach can handle complex scenarios with multiple state changes, enabling recognition of states that do not follow a simple, one-way transition (\eg multiple simultaneous transition).
(iii) \textbf{Avoiding Ambiguity}: Pre-defining state classes in text reduces ambiguity by clearly delineating what each state entails, ensuring consistency in classification.


% 状態の意味について柔軟にその定義に基づいてラベリングするのは難しい．
The challenge of this task is to collect multi-label training data tailored to object state definitions. Manual annotation of temporally changing multiple object states (\eg \cite{liu2017jointly}) requires a lot of exhausting work and is vulnerable to changes in vocabulary and definition.
To bypass the annotation effort, we propose a framework that uses large language models (LLMs) to create object state pseudo-labels based on narrations in instructional videos (Figure \ref{fig:teaser}). Narrations offer valuable information about what is happening in visual content and can be used as a scalable resource for training models. Our observation is that the sequence of past actions extracted from video narrations tells about when an object state appears and disappears.
Given the narration, our framework first extracts action information and then leverages cause-and-effect knowledge encoded in LLMs to describe the resulting state after each action. The inferred sequence of state descriptions tells what effects have been caused to the object. Finally, we use this sequence of descriptions to consider context to infer the state labels at each moment of the video.

% Specifically, we introduce context-aware pseudo-labeling that considers all the past state changes of the object, allowing the framework to infer multiple aspects of object states.
% For example, after peeling, slicing, and grating the apple, the state is no longer {\it sliced} because the apple lost the distinct shape of the slice. We also use vision-language models (VLMs) to temporally align the inferred object state labels and video frames. 
% To bypass the annotation effort, we explore learning from instructional videos on the Internet with automatically transcribed narrations. Narrations offer valuable information about what is happening in visual content and can be used as a scalable resource for training models.
% is adopted in various video recognition tasks~\cite{alayrac2016unsupervised,miech2020end,bertasius2020cobe}.
% Narrations in instructional videos offer valuable information about what people do in the videos and can be used as a scalable resource for training models. 
% 課題の提示：物体状態はナレーション内で述べられていない
% However, learning object states directly from video narrations would not be successful because (i) narrations mostly mention what they are doing and less describe object states, and (ii) narrations don't tell when a certain object state is positive or negative based on the definition.
% has not been as successful as learning actions and objects.
% In instructional videos, speakers talk about the most important events first, and often omit obvious or unimportant information~\cite{gordon2013reporting,misra2016seeing}.
% They often do not tell much about the states of objects compared to what they are doing (actions) and what they are handling (objects).
% Therefore, naively training recognition models for less described entities from raw narrations may lead to suboptimal results.

% 問題提起：ナレーションに暗黙的に含まれる状態を引き出すことはできないだろうか？
% How can we utilize the untold object state information implicitly told in narrations and create labels for training?
% We propose to use off-the-shelf large language models (LLMs) to infer the object states from action information included in video narrations (Figure~\ref{fig:teaser} left).
% % （八木）LLMは言い換えに優れる
% LLMs trained by massive amounts of text corpus are showing impressive reasoning abilities in various tasks~\cite{gpt-3,bubeck2023sparks}.
% They are especially good at re-arranging information such as summarization~\cite{witteveen2019paraphrasing} and paraphrasing~\cite{witteveen2019paraphrasing}.

% Our key idea is to infer the presence of object states from video narrations by LLMs from the actions described in video narrations.
% We argue that the sequence of past actions extracted from video narrations tells about when an object state appears and disappears.
% For example, after peeling, slicing, and grating the apple, the state is no longer {\it sliced} because the apple lost the distinct shape of the slice.
% The relationship between actions and object states implicitly encoded in LLMs allows us to generate pseudo-object state labels.
% for training a frame-wise object state classification model. 
% 手法の大枠：ナレーションから行動への抽出→行動から状態の推論→疑似ラベルとして訓練
% Specifically, we propose a three-step framework to infer temporally localized object state information from video narrations.
% First, given transcribed narrations with a target object category name, we extract a set of {\it manipulation actions} describing the actions related to target objects.
% Next, for each primary action, we generate its {\it state descriptions} which describes the resulting states caused or inferred by that specific action.
% Finally, the accumulated list of inferred state descriptions is used to determine the presence of a specific object state at each time.
% LLMs are used in each phase to bridge between the above concepts.
% 時刻との対応付けを取る


% Xue et al.やその他との比較 TODO
Concurrently to our work, Xue \etal \cite{xue2023learning} propose to use LLMs to find specific object state changes from internet video narrations and use VLMs to localize different states (\textit{initial}, \textit{transitioning}, and \textit{end}) in videos, creating pseudo-labels for training. However, it is worth noting that our framework is different in that it tackles the unique difficulty of the multi-label problem: It requires (i) considering the whole past context of multiple object state changes and (ii) capturing more implicit object state information indicated by the actions, to infer multiple object states at each moment.

% self-training
% The generated object state labels are used to train a frame-wise classification model.
% However, the generated labels are temporally sparse due to the ambiguity of action information, which we found leads to incorrect learning of temporal context.
% To address the issue of unlabeled segments, we introduce a self-training scheme where a trained teacher model labels the unlabeled segments, allowing a student model to train on fully labeled data.
% In particular, we introduce the use of two models with different context lengths as teacher models and employ an ensemble approach to supervise the student model. To the best of our knowledge, this is the first application of self-training from an ensemble to learn from temporally partially labeled data, demonstrating the efficacy of combining individual frame features and temporal context.

% 実験とMOSTデータセットの導入
Since there are no suitable datasets evaluating the temporal segmentation performance of multi-label object states, we collected a new Multiple Object States Transition (MOST) dataset containing 60 object states from six object categories (apple, egg, flour, shirt, tire, and wire).
The MOST dataset is designed to evaluate finding the presence of object states, different from the previous datasets~\cite{look_for_the_change,grauman2022ego4d,xue2023learning}, which aim to find the different phases of object state change.
% MOST dataset exhibits far more dense annotation compared to the previous dataset~\cite{look_for_the_change,grauman2022ego4d} 
Experimental evaluation showed that our model demonstrates significant improvement of over 29\% in mAP against strong zero-shot vision-language models~\cite{clip,wang2022internvideo}, suggesting the effectiveness of explicitly extracting object state information implicit in narrations, through LLMs.
It also achieved competitive performance in localizing state-changing actions in the ChangeIt dataset~\cite{look_for_the_change} with minimum modifications.

% 貢献の記述
% Our contributions are as follows:
% \begin{itemize}
%     \item We reformulate object state recognition as a multi-label frame-wise classification task and explicitly address the range of each state.
%     \item We propose a flexible framework that generates pseudo-labels for the presence of object states based on action information from narrations using LLMs and train the model accordingly.
%     \item We construct an evaluation dataset and achieve higher performance compared to existing strong vision-language models.
% \end{itemize}



==> sec/3_method_old.tex <==
\section{Method}
\label{sec:method}

\subsection{Problem Setting}
\label{subsec:problem_setting}
Our goal is to predict the existence of multiple object states at each moment of a video.
Therefore, we formulate the problem as a multi-label frame-wise classification task.

Formally, we assume a set of instructional videos $\mathbf{X} \in \mathcal{V}$ including the object of interest with multiple object state changes.
Each video is accompanied by a set of video narrations describing the content of the video.
Given a video $\mathbf{X}=\{\mathbf{x}_1, \mathbf{x}_2, \dots, \mathbf{x}_T\}$ of length $T$, the goal is to predict a sequence of binary vectors $\mathbf{Y} = \{\mathbf{y}_1, \mathbf{y}_2, \dots, \mathbf{y}_T\}$, where $\mathbf{y}_i = \{y_i^1, y_i^2, ..., y_i^K\}$ is a binary vector denoting the presence of $K$ object state labels at time $i$.

Since there is often a range of meanings for an object state, we assume pairs of a state name (\eg, sliced) and its textual definition composed of a few sentences (\eg, ``the state of an apple that has been cut into thin or narrow pieces. It does not include the case where the apple is split into two or three large pieces. Even if it is cooked, it is still applicable as long as it retains the shape of the pieces.'').
Object state labels are not mutually exclusive and more than one object state may appear in a video frame simultaneously (\eg, a shirt may be {\it soaked} and {\it dyed} at the same time).

% LLMに基づくナレーションからの物体状態情報抽出
\subsection{Object State Label Extraction from Actions via LLMs} % 八木案
\label{subsec:object_state_inference}
To address the lack of object state information in video narrations, we introduce a three-stage framework for generating object state multi-labels from video narrations via LLMs, namely consisting of (a) manipulation action extraction (b) state description generation from actions (c) context-aware object state label inference.
The key observation is that the presence of each object state, which is not necessarily mentioned in the narrations, can be inferred from (1) the actor's current actions and (2) the past object state of the object.
We leverage LLMs at each stage to efficiently derive object state information from noisy narrations.

The key difference between our framework and the previous work \cite{xue2023learning} that uses LLMs to find specific state-modifying actions and VLMs to discriminate different states is that our framework aims to exploit whole past context of object state changes by producing intermediate state descriptions to efficiently and effectively derive multiple state information.


\begin{figure*}[tb]
    \centering
    \includegraphics[width=1\linewidth]{fig/llm_part.pdf}
    \caption{Three-stage framework of inferring presence of object state labels from video narration. (a) Manipulation action extraction from narration. (b) Object state description generation from actions. (c) Context-aware object state label inference.}
    \label{fig:llm_part}
\end{figure*}

\subsubsection{Manipulation Action Extraction} % 八木案
The goal of this stage is to extract a set of manipulation actions of the actor from ASR narrations.
Raw ASR transcriptions accompanied with instructional videos offer valuable information on the actor's actions.
However, raw narrations often contain transcription errors, over-segmentation, and irrelevant contents unrelated to the visible actions which may harm inferring object states.
To this end, we first leverage LLMs to extract {\it manipulation actions} that the actor actually conducts in the scene, from narrrations (See supplementary for full prompts).
Specifically, a small block of narrations and their timestamps (10 sentences per block) are fed into LLMs to output a set of manipulation actions. (Figure~\ref{fig:llm_part} (a))
Note that manipulation actions do not correspond to original narrations one by one.
To obtain the time interval for each extracted action, we also prompt LLMs to refer back to mark the narration that best match what the action says, and take the interval of it as the interval of the manipulation action.

\subsubsection{Object State Description Generation from Actions}
Next, we sequentially generate a set of {\it state description} from manipulation actions, which is used as intermediate information before generating the multi-label object state pseudo-labels (Figure~\ref{fig:llm_part} (b)).
State description is a short sentence including the target object name and a description concisely describing their state.
The motivation of state description is to keep track of the object's state at that time while (i) detecting whether the object has undergone any kind of state change and (ii) dealing with changes in the object name.

% メカニズムを先に書いてみる
In this stage, we assume a set of action blocks, each including 10 manipulation actions, and the initial state description is set as ``The state of $<$object name$>$ is unknown.''.
At each block, we pass the set of current manipulation actions and the last state description to LLMs and generate a sequence of state descriptions corresponding to each action.
By considering the past state description, LLMs can track what change has been applied to the object, and generate temporally consistent state descriptions across videos.

We found that explicitly generating the current object name is crucial in this case because the names of the objects often change as a result of object state changes.
For example, a sliced apple mixed with other ingredients would be later called a {\it mixture} in some narrations.
In such a case, it is no longer called as {\it apple} anymore.
Therefore, an explicit mechanism to infer that the {\it apple} has changed to a {\it mixture} is necessary to keep track of the object state changes.


\subsubsection{Context-aware Object State Label Inference}

Finally, we infer whether a target object state (\eg, whole, cooked, or sliced) is present at the timing of each state description. (Figure~\ref{fig:llm_part} (c))
For each state description, we feed the concatenation of all the state descriptions up to that timing to LLMs and prompt it to produce the presence (in either ``Yes'', ``No'' or ``ambiguous'') of each of the $K$ object states.
Because some object states are kept unchanged from the beginning of the video, it is crucial to input all their temporal context.
Since target object state names are often not enough to determine their meanings, we also input their detailed definition to LLMs.
We allow LLMs to answer ``ambiguous'' if the given list of state descriptions does not contain enough information.
The object state labels determined as ambiguous are not used for training.

\subsection{Interval Alignment via VLMs}
\label{subsec:aligning_object_states}

We now obtained a list of object state labels with their corresponding manipulation actions and time intervals.
The intervals of actions roughly correspond to the presence of the object states.
However, they are not correctly temporally aligned due to misalignment between (a) narrations and video frames (b) the presence of object states and actions.
Therefore, there is a need to match between object states and video frames.
Instead of explicit alignment (\eg, \cite{dvornik2023stepformer}) we introduce a simple two-stage technique of assigning object state labels to video frames, using off-the-shelf vision-language models (VLMs).

Figure \ref{fig:alignment} shows the detailed procedure. 
Similar to Sec.~\ref{subsec:object_state_inference}, our observation is that the interval of an object state roughly matches with that of its corresponding action.
First, given a video frame, we ask the VLM the most plausible manipulation action to the frame from candidate manipulation actions within before/after $\Delta t$ seconds around the frame (Figure~\ref{fig:alignment} (a)).
We allow the VLM to choose ``others'' option if no actions represent the frame.
The frame is not used for training if ``others'' is chosen.

Once we assign likely actions to each frame, we then use the corresponding object state description to filter out irrelevant frames using VLMs (Figure~\ref{fig:alignment} (b)).
We assign object state labels with their value (true/false) to the video frames that passed this phase.

Note that determining intervals by looking at the action does not mean that pseudo-labels are assigned only if state-changing actions exist.
We can infer the presence of object states from some actions not related to their state change.
For example, ``picking apples from the tree'' implies that the apples are whole and not sliced or cooked even though it does not trigger object state changes.


\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{fig/alignment.pdf}
    \caption{Temporal alignment between video frames and action/object state description pair. (a) Given video frame, we select most likely actions from surrounding candidates using VLMs. (b) Interval is further filtered by matching frame and state description.}
    \label{fig:alignment}
\end{figure}


\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{fig/self_training.pdf}
    \caption{Self-training via ensemble of teacher models.} 
    \label{fig:self-training}
\end{figure}

\subsection{Learning from Pseudo-Object State Labels: Self-Training from Ensemble}
\label{subsec:learning_object_states}
Finally, we train the frame-wise object state classifier using generated pseudo-object state labels.
% \subsubsection{Pseudo-Label Preprocessing}
% To make the model sensitive only to visible target objects, we use CLIP~\cite{clip} to assign negative labels to the frames without target objects.
% We take the cosine similarity between a video frame and pre-defined target object names and assign negative labels to all the object states if their maximum score is under a certain threshold.
% \subsubsection{Self-Training from Ensemble}
However, the generated pseudo-labels are partially assigned to video frames.
While we would like to employ temporal models to capture the dynamics between actions and object states, directly learning from the partial pseudo-labels results in suboptimal results.
Therefore, we introduce a self-training scheme based on mean teacher learning~\cite{tarvainen2017mean} which updates the target student model from the ensemble of teacher models initialized from pseudo-labels.

Our key idea is that we can fill the unlabeled segments by efficiently propagate the the knowledge learned from labeled segments using two different models. Figure~\ref{fig:self-training} shows the overview of training.
We first train two frame-wise {\it teacher} state classification models with different temporal windows: {\bf MLP} and {\bf TCN}, using the original pseudo-labels. The idea behind using two different temporal context models is that object states can be predicted both from frame-wise object appearance and temporal action context, which are complementary in object state recognition.

% TODO
Both models have a pre-trained backbone fixed during training and additional layers for fine-tuning.
while they are similar to action segmentation models (\eg, \cite{farha2019ms}), the final layer of each model has a sigmoid activation because object states are not mutually exclusive.
They are trained with standard binary cross entropy loss only calculated for valid pseudo-labels. % weighted bce

In this work, we use the InvernVideo~\cite{wang2022internvideo} visual encoder for the backbone.
{\bf MLP} has a 2-layer MLP head and it does not take any temporal context into account.
{\bf TCN} has stacked temporal convolutional networks to model the temporal relationship between frames.
We modify MS-TCN~\cite{farha2019ms} to replace the softmax layer in each stage with a sigmoid layer.
At this phase, {\bf TCN} does not perform well due to missing pseudo-labels.


Given the above two models as teacher models, we propose to train another set of {\bf MLP} and {\bf TCN} as student models, taking the weighted sum of teacher models' predictions as ground truth.
The ensemble of two soft labels mitigates the missing label issue on training the student {\bf TCN} model.
Formally, the new ensembled target $\mathbf{y_t^{ens}}$ for $t$-th video frame can be denoted as follows:
\begin{align}
\mathbf{y_t^{ens}} = \mathbf{\alpha \cdot \hat{y}_t^{TCN}}+ (1-\alpha) \cdot \mathbf{\hat{y}_t^{MLP}}.
\end{align}
where $\mathbf{\hat{y}_t^{TCN}}$ and $\mathbf{\hat{y}_t^{MLP}}$ are the output of {\bf MLP} and {\bf TCN}, respectively, and $\alpha \in [0, 1]$ denote the weight of different labels.
In this work, we set $\alpha$ to 0.5.

Following the mean teacher strategy~\cite{tarvainen2017mean,han2022temporal}, we concurrently update the parameters of the teacher models via the Exponential Moving Average (EMA) mechanism.
The teacher models are gradually updated to follow the student models.
We use the momentum coefficient of 0.999.
After student model training, only the student {\bf TCN} model is used for inference.

==> sec/4_experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

We examine our proposed approach in two benchmarks: Newly collected Multiple Object States Transision (MOST) dataset and the existing ChangeIt dataset~\cite{look_for_the_change}.


\subsection{Multiple Object States Transition Dataset (MOST)}
\label{subsec:dataset}

Since there were no publicly available datasets on temporally localizing the presence of object states, we created a new evaluation dataset called Multiple Object States Transition (MOST) dataset.
We manually collected instructional videos from YouTube for six object categories: apple, egg, flour, shirt, tire, and wire, that take various types of object states.
We selected around 10 object states per object category to annotate, covering the popular states the object may take (see supplementary for full lists).
For the videos showing the target object, annotators marked the interval where each object state exists.
As a result, 61 videos with a total duration of 159.6 minutes were fully annotated.


% \begin{figure}[tb]
%   \centering
%   \begin{subfigure}{0.5\linewidth}
%   \includegraphics[width=1\linewidth]{fig/most_ex_1.pdf}
%     \caption{Scene: Cooking food with flour.}
%     \label{fig:most_ex_1}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.49\linewidth}
%   \includegraphics[width=1\linewidth]{fig/most_ex_2.pdf}
%     \caption{Scene: Washing car tire.}
%     \label{fig:most_ex_2}
%   \end{subfigure}
%   \caption{Annotation example of MOST dataset. Red bands show presence of object states by time (seconds). All labels are marked negative if target objects are not visible.}
%   \label{fig:annotation_example}
% \end{figure}
\begin{figure}[tb]
  \centering
  \begin{subfigure}{1\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/most_ex_1.pdf}
    \caption{Scene: Cooking food with flour.}
    \vspace{.5cm}
    \label{fig:most_ex_1}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{fig/most_ex_2.pdf}
    \caption{Scene: Washing car tire.}
    \label{fig:most_ex_2}
  \end{subfigure}
  \caption{Annotation example of MOST dataset. Red bands show presence of object states by time (seconds). All labels are marked negative if target objects are not visible.}
  \label{fig:annotation_example}
\end{figure}

% 先行データセットとの違い：
As shown in the examples (see Figure~\ref{fig:annotation_example}), the object states are densely annotated, and have more complicated transition patterns between different states to measure when the object state is actually present rather than finding the timing of state-changing actions as in previous datasets~\cite{joint_discovery,look_for_the_change}.

Indeed, ChangeIt~\cite{look_for_the_change} annotates object state labels as pre/post condition of actions.
For example, the \textit{initial} label for \textit{Cake frosting} is only marked just before the action starts, but the frames of unfrosted cake that are temporally distant from the action are labeled as \textit{background}, which means that the presence of object states cannot be determined solely without state-changing actions.

The MOST dataset covers various object states including those that are not necessarily associated with actions (\eg, straight, dry, flat, smooth), providing a more direct benchmark of object state recognition.

\subsection{Implementation Details}
\label{subsec:implementation}
\subsubsection{Training Data}
We used the subset of HowTo100M~\cite{howto100m} as training data.
We assume access to the target object names and their states to recognize.
Given a target object name (\eg, apple), we first selected videos that included the object name in the title and narration.
We further selected videos that included the verbs likely to be associated with the target objects.
We used LLMs to automatically create a list of the likely associated verbs.
For example, from an object-state pair ``peeled apple'', verbs such as ``peel'', ``slice'', and ``cut'' are suggested.
Finally, we removed videos with very long narrations ($>$ 12,000 words) to fit the maximum context length of LLMs, resulting in around 2K videos per object category by adjusting the maximum YouTube search rank (see supplementary for details).

For evaluation of ChangeIt dataset \cite{look_for_the_change}, we used the subset of the original ChangeIt videos including narrations for training.
We selected at most 350 videos per category with the highest noise adaptive weight~\cite{look_for_the_change}.
This results in 10,749 videos in total, which is 32\% of the original dataset. 


\subsubsection{Pseudo-Label Generation}
We used the pre-processed narrations from \cite{han2022temporal} that removed low-quality subtitles.
We used GPT-3.5 (\texttt{gpt-3.5-turbo-1106}) for the LLM to process narrations.
Samples that did not follow the specified output format (approximately 1\%) are discarded.
We used LLaVA-1.5 13B \cite{liu2023improved} 4-bit quantized model for VLMs used for temporal alignment.
We set the window $\Delta t$ to 10 seconds on selecting manipulation action candidates.

We applied our framework to videos of 1,123 hours in total.
As a result, pseudo-labels are assigned to 74\% of the video frames.

\subsubsection{Models}
For the feature backbone, we used the pre-trained InternVideo visual encoder (InternVideo-MM-14-L)~\cite{wang2022internvideo} and sampled 8 frames per second to obtain the feature vectors at 1~fps.
For the {\bf TCN} classifier, we used MS-TCN~\cite{farha2019ms} with 4 stages.
Each stage consists of 10 layers of 512 dimensions, followed by a final linear layer of $K$ outputs with Sigmoid activation.
The {\bf MLP} classifier is a simple MLP consisting of a linear layer of 512 dimensions followed by ReLU activation and the final linear layer of $K$ outputs followed by Sigmoid activation.
The models were trained separately for each object category.


\subsubsection{Optimization}
We have two learning stages: one for learning the teacher models using pseudo-labels generated by LLMs and the other for self-training with the student model. We train each model with a batch size of 16 for 50 epochs in the first stage, followed by 50 epochs in the second one. We use the Adam optimizer~\cite{kingma2014adam} with decoupled weight decay regularization~\cite{loshchilov2017decoupled}. We set the learning rate to 1e-4 and the weight decay to 0.01.

\subsubsection{Datasets and Metrics}


For MOST dataset, we report F1-max and Average Precision (AP) to measure the correctness of temporal localization of object states.
To make scores comparable against uncalibrated zero-shot models, we report F1-max which is the maximum F1 score at the optimal threshold.
We set the thresholds for each object state category.

ChangeIt dataset evaluates the performance of temporally localizing (i) the initial state, (ii) the state-modifying action, and (iii) the end state.
For 44 state-changing actions, 667 videos up to 48 hours are annotated for evaluation.
Following \cite{look_for_the_change} we report precision@1 for action and state respectively.

\subsection{Evaluation on MOST Dataset}
\label{subsec:results_most}

\subsubsection{Comparison to off-the-shelf VLMs}
To show the effectiveness of explicitly generating object state labels from narrations via LLMs, we compared our method with three zero-shot VLM models trained from various vision-language data: LLaVA~\cite{liu2023improved}, CLIP~\cite{clip}, and InternVideo~\cite{wang2022internvideo}.

% ここからLLaVAの説明
LLaVA is a large multi-modal LLM that accepts a pair of an image and texts.
We used the same model (LLaVA-1.5 13B 4-bit quantized) which is used in interval alignment of our proposed method.
We feed each video frame and object state definition to LLaVA and prompt it to first describe the image and then answer whether the object state is present in the image.
As the model only produce binary predictions, we only compute the F1-max score.

% ここからCLIPの説明
CLIP~\cite{clip} is a simple yet strong model trained by massive image-text pairs with contrastive learning.
We input each video frame and object state text to the image and text encoder to calculate the similarity score between frames and object states.
Similar to \cite{look_for_the_change}, we tested several text prompts such as ``a photo of \textless object state\textgreater \textless object name\textgreater'' (\eg, ``a photo of cracked egg'') and reported their best results (see supplementary for details).

InternVideo~\cite{wang2022internvideo} is a video-language foundation model based on masked video reconstruction and multi-modal contrastive learning, demonstrating strong results on various video recognition tasks.%, especially on action understanding and video-text retrieval task.
We input the model 8 video frames and the object state text similar to CLIP.

%TODO object state textを適切なものに変える

Table \ref{tab:comparison_sota} shows the quantitative results.
Our method achieves significantly better results and outperforms all the strong zero-shot baselines in both F1-max and AP, showing the effectiveness of learning from LLM-based object state pseudo-labels.

\begin{table*}[tb]
    \centering
    \caption{Comparison with other baselines on MOST dataset. F1 denotes F1-max score and mAP denotes mean Average Precision score averaged across object state categories.}
    \scalebox{0.9}{
    \begin{tabular}{lcccccccccccccc}
    \toprule
      Method & \multicolumn{2}{c}{Apple} & \multicolumn{2}{c}{Egg} & \multicolumn{2}{c}{Flour} & \multicolumn{2}{c}{Shirt} & \multicolumn{2}{c}{Tire} & \multicolumn{2}{c}{Wire} & \multicolumn{2}{c}{{\bf Average}} \\
      \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
      & F1 & mAP & F1 & mAP & F1 & mAP & F1 & mAP & F1 & mAP & F1 & mAP & F1 & mAP \\
    \midrule      
      LLaVA~\cite{liu2023improved} & 0.34 & \NA & 0.29 & \NA & 0.35 & \NA & 0.28 & \NA & 0.47 & \NA & 0.27 & \NA & 0.33 & \NA \\
      CLIP~\cite{clip} & 0.42 & 0.35 & 0.37 & 0.28 & 0.38 & 0.26 & 0.33 & 0.27 & 0.55 & 0.45 & 0.33 & 0.25 & 0.39 & 0.31 \\
      InternVideo~\cite{wang2022internvideo} & 0.46 & 0.39 & 0.44 & 0.39 & 0.43 & 0.36 & 0.40 & 0.32 & 0.57 & 0.45 & 0.40 & 0.31 & 0.45 & 0.37 \\
      \textbf{Ours} & \textbf{0.53} & \textbf{0.50} & \textbf{0.53} & \textbf{0.48} & \textbf{0.55} & \textbf{0.49} & \textbf{0.50} & \textbf{0.45} & \textbf{0.61} & \textbf{0.52} & \textbf{0.50} & \textbf{0.42} & \textbf{0.54} & \textbf{0.48} \\
  \bottomrule
\end{tabular}
}
\label{tab:comparison_sota}
\end{table*}




\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{fig/qualitative_apple.pdf}
    \caption{Qualitative results of proposed model (target object: apple). Blue and red bar denote our model's prediction and ground truth, respectively.}
    \label{fig:qualitative}
\end{figure}

\subsubsection{Qualitative Analysis}
Figure \ref{fig:qualitative} shows the predictions of our trained model.
Blue and red bar denote the prediction and the ground truth labels, respecitvely. 
Overall our model correctly localize the presence of mulitple object states while there are false positive predictions in some labels (\eg, sliced, cooked).


\subsection{Ablation Study}

\subsubsection{Does temporal context matter in pseudo-label generation?}
We compare the model trained with pseudo-object state labels without using temporal context (Table~\ref{tab:ablation} top).
In this model, we infer the state description and the object state labels each from single manipulation action one-by-one.
We observe 3\% gain on mAP showing that temporal context matters in inferring object states from actions.
In Figure \ref{fig:ablation_no_context}, we show an example of incorrect label generation due to a lack of context information.
Figure~\ref{fig:ablation_results_context} shows that models trained with context-aware labels produce better predictions. 

\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{fig/no_context.pdf}
    \caption{Effect of temporal context on object state label inference. Action ``Observing coagulation'' tells only that egg is changing from unsolidified to solidified state, but it lacks other information such as whether egg is in shell or broken. These lack of information often leads to incorrect reasoning (top). This issue is mitigated by taking past history of actions into account (bottom).}
    \label{fig:ablation_no_context}
\end{figure}

\begin{figure}[tb]
  \centering
  \begin{subfigure}{0.47\linewidth}
  \includegraphics[width=1\linewidth]{fig/context_result.pdf}
    \caption{Comparison of prediction results between models trained by pseudo-labels with and without temporal context.}
    \label{fig:ablation_results_context}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.52\linewidth}
  \includegraphics[width=1\linewidth]{fig/self_result.pdf}
    \caption{Effect of self-training. Bar with darker colors mean high probability for the former three models. The blue and red bars denote prediction of self-trained model and ground truth labels. MLP and MS-TCN denote models trained without self-training.}
    \label{fig:ablation_results_self}
  \end{subfigure}
  \caption{Qualitative analysis on the impacts from our key component. (a) Pseudo-labels generated w/o considering temporal context lead to false positive (top) and false negative (bottom) predictions due to incorrect label assignment. (b) The self-training model inherits the best aspects of both the MLP and MS-TCN models.}
  \label{fig:Qualitative results for ablation study.}
\end{figure}

\subsubsection{Is self-training effective?}
Table~\ref{tab:ablation} middle shows the performance of {\bf TCN} and {\bf MLP} models directly trained from pseudo-labels.
While {\bf TCN} trained from raw pseudo-labels shows inferior results against {\bf MLP}, its performance surpasses {\bf MLP} by 3\% after self-learning.
Figure~\ref{fig:ablation_results_self} comparison against a video of {\it a wire twisted}.
The final model suppresses the errors of the two teacher models.

\subsubsection{Does action/state alignment help?}
As shown in Table~\ref{tab:ablation} bottom, action/state alignment using VLMs showed a marginal improvement of 2\%.

\begin{table}
    \centering
    \caption{Ablation results.}
    \begin{tabular}{lcc}
    \toprule
    %\multirow{2}{*}{Method} & \multicolumn{2}{c}{Average} \\
      %\cmidrule(lr){2-3} &
      %F1-max & mAP \\
      Method & F1-max & mAP \\
    \midrule
        Full model & \textbf{0.54} & \textbf{0.48}\\
        w/o context-aware pseudo-labels & 0.52 & 0.45\\
        w/o self-training (MS-TCN) & 0.44 & 0.36\\
        w/o self-training (MLP) & 0.51 & 0.45\\
        w/o action/state alignment & 0.53 & 0.46\\
    \bottomrule
    \end{tabular}
    \label{tab:ablation}
\end{table}

\subsection{Evaluation on ChangeIt Dataset}
\label{subsec:results_changeit}

%\subsubsection{Training Setup}
Since the problem is different from that of MOST dataset, we made minor modifications to produce the three labels ({\it initial state}, {\it action}, and {\it end state}) during pseudo-label generation.
We assign {\it background} label to video frames without a target object as in Section \ref{subsec:learning_object_states}.
% We compute the optimal threshold for assigning \textit{backgorund} label and report the best value.
Due to high computational demands, we omit the matching between state description and video frames.
For a fair comparison, we also use the causal ordering constraints~\cite{look_for_the_change} at inference by selecting the frames of \textit{initial state}, \textit{action}, and \textit{end state} with their highest probabilities while respecting their causal order.

%\subsubsection{Results}
Table~\ref{tab:comparison_changeit} shows the results.
Although our method uses less training data (approx. 30\%), our method achieves competitive performance against the best single-task learning model~\cite{look_for_the_change}, without relying on the strong heuristics of causal ordering constraints during training.
%Our method prioritizes learning object states, which results in a compromise on action recognition capabilities.

%We test our method on ChangeIt \cite{look_for_the_change} dataset. When creating pseudo-labels from narrations using LLMs, we can basically use the same method and prompts as described in Section \ref{sec:method}. However, we introduced a minor modification to the prompts to facilitate the selection among three potential labels: {\it initial state}, {\it action}, and {\it end state} based on a list of state descriptions. We assign {\it background} label to video frames where an object in focus isn't present in the same way as in Section \ref{subsec:learning_object_states}. We compute the optimal threshold for assigning \textit{backgorund} label and report the best value. Due to the high computational demands, we bypass the explicit assignment of state descriptions and instead, automatically assigned the state description to all frames where the corresponding action is identified. For a fair comparison with previous works, we apply the causal ordering constraints~\cite{look_for_the_change} in the inference stage where we select the frames of \textit{initial state}, \textit{action}, and \textit{end state} with the highest probability such that those three labels are arranged in the order \textit{initial} $\rightarrow$ \textit{action} $\rightarrow$ \textit{end}

\begin{table}[tb]
  %\caption{Comparison on ChangeIt dataset. For state precision@1, our method outperforms previous works using only 32\% of training data in ChangeIt dataset. Our method prioritizes learning object states, which results in a compromise on action recognition capabilities.}
  \caption{Comparison on ChangeIt dataset. The rightmost two columns show precition@1 for states and actions, respectively.}
  \centering
  \begin{tabular}{lp{3.6cm}cc}
    \toprule
    Method & Training Data & State prec. & Action prec. \\
    \midrule
    \textbf{\textit{Single task models}} & & \\
    %\multicolumn{3}{l}{\textbf{\textit{Single task formulation}}} \\
    Random w/ constraint & \NA & 0.15 & 0.41 \\
    CLIP ViT-L/14 \cite{clip} & Zero-shot & 0.30 & 0.63 \\
    Alayrac \etal \cite{alayrac2016unsupervised} & ChangeIt (full) & 0.30 & 0.59 \\
    Look for the Change \cite{look_for_the_change} & ChangeIt (full) & 0.35 & 0.68 \\
    \textbf{Ours} & ChangeIt (w/\.narration) & 0.42 & 0.56 \\
    \midrule
    \multicolumn{3}{l}{\textbf{\textit{Multi-task models}}} \\
    Multi-Task  \cite{multi_task}  & ChangeIt (full) & 0.49 & 0.80 \\
   \bottomrule
  \end{tabular}
\label{tab:comparison_changeit}
\end{table}

